The Occurrence Rate of Quiescent Radio Emission for Ultracool Dwarfs using a Generalized Semi-Analytical Bayesian Framework

We present a generalized analytical Bayesian framework for calculating the occurrence rate of steady emission (or absorption) in astrophysical objects. As a proof-of-concept, we apply this framework to non-flaring quiescent radio emission in ultracool ($\leq$ M7) dwarfs. Using simulations, we show that our framework recovers the simulated radio occurrence rate to within 1-5% for sample sizes of 10-100 objects when averaged over an ensemble of trials and simulated occurrence rates for our assumed luminosity distribution models. In contrast, existing detection rate studies may under-predict the simulated rate by 51-66% because of sensitivity limits. Using all available literature results for samples of 82 ultracool M dwarfs, 74 L dwarfs, and 23 T/Y dwarfs, we find that the maximum-likelihood quiescent radio occurrence rate is between $15^{+4}_{-4}$ - $20^{+6}_{-5}$%, depending on the luminosity prior that we assume. Comparing each spectral type, we find occurrence rates of $17^{+9}_{-7}$ - $25^{+13}_{-10}$% for M dwarfs, $10^{+5}_{-4}$ - $13^{+7}_{-5}$% for L dwarfs, and $23^{+11}_{-9}$ - $29^{+13}_{-11}$% for T/Y dwarfs. We rule out potential selection effects and speculate that age and/or rotation may account for tentative evidence that the quiescent radio occurrence rate of L dwarfs may be suppressed compared to M and T/Y dwarfs and phenomenon. Finally, we discuss how we can harness our occurrence rate framework to carefully assess the possible physics that may be contributing to observed occurrence rate trends.

==> TABLE_simulation_20Nobs.tex <==
\setlength{\tabcolsep}{0.05in}
\begin{deluxetable*}{ccccrrccllll}[htp]
\tabletypesize{\scriptsize}
\tablecaption{Summary of mean simulation results for N = 20 \label{ table:simulation_20Nobs } } 
\tablehead{
\colhead{ }   	&
\colhead{ }		&
\colhead{ }   	&
\colhead{ } 		&
\colhead{ }   	&
\colhead{ } 		&
\colhead{ }   	&
\colhead{ } 		&
\multicolumn{2}{l}{$\theta_{\mathrm{emit}}$ recovery rate}  &
\multicolumn{2}{l}{$\theta_{\mathrm{true}}$ recovery rate} \\[-9pt] 
% 
\colhead{$\hat{\theta}_{\mathrm{true}}$}   		&
\colhead{$\hat{\theta}_{\mathrm{emit}}$}		    &
\colhead{$\hat{\theta}_{\mathrm{calc}}$}   		&
\colhead{$\hat{\theta}_{\mathrm{detect}}$} 		&
\colhead{$\mid \hat{\epsilon}_{\mathrm{calc}} \mid$}   		&
\colhead{$\mid \hat{\epsilon}_{\mathrm{detect}} \mid$} 		&
\colhead{$\hat{f}_{\mathrm{calc}}$}   		&
\colhead{$\hat{f}_{\mathrm{detect}}$} 		&
\colhead{$\theta_{\mathrm{calc}}$ CI} 	&
\colhead{$\theta_{\mathrm{detect}}$ CI} 	&
\colhead{$\theta_{\mathrm{calc}}$ CI} 	&
\colhead{$\theta_{\mathrm{detect}}$ CI} \\[-9pt] 
% 
\colhead{(\%)}  				& 
\colhead{(\%)}  				& 
\colhead{(\%)}  				& 
\colhead{(\%)}  				& 
\colhead{(\%)}	  				& 
\colhead{(\%)}  					& 
\colhead{ }	  				& 
\colhead{ }  					& 
\colhead{(\%)}  				& 
\colhead{(\%)}  				& 
\colhead{(\%)}  				& 
\colhead{(\%)}  				\\[-9pt] 
% 
\colhead{ }   	&
\colhead{ }		&
\colhead{ }   	&
\colhead{ }   	&
\colhead{ } 		&
\colhead{ }   	&
\colhead{ } 		&
\colhead{ } 		&
\colhead{ 68.3, 95.5, 99.7}	&
\colhead{ 68.3, 95.5, 99.7}	&
\colhead{ 68.3, 95.5, 99.7}	&
\colhead{ 68.3, 95.5, 99.7}  
}	
\startdata
 10.0  &  9.8 &  $9.5_{-5.8}^{+17.1}$ & $3.3_{-2.7}^{+2.7}$  &    4.5 & 67.0   &    $1.0_{-0.7}^{+1.6}$ & $3.0_{-1.3}^{+13.6}$   &   90.0, 100.0, 100.0    &   42.0, 57.0, 64.0  &   87.0, 99.0, 100.0   &    50.0, 50.0, 50.0  \\[3pt] 
 20.0  &  19.1 &  $17.7_{-9.0}^{+18.4}$ & $6.1_{-3.8}^{+3.8}$  &    11.6 & 69.5   &    $1.1_{-0.6}^{+1.2}$ & $3.3_{-1.3}^{+5.6}$   &   69.0, 99.0, 100.0    &   25.0, 42.0, 54.0  &   56.0, 98.0, 100.0   &    18.0, 46.0, 64.0  \\[3pt] 
 30.0  &  31.4 &  $30.0_{-13.4}^{+19.5}$ & $10.1_{-5.6}^{+5.6}$  &    0.1 & 66.3   &    $1.0_{-0.4}^{+0.8}$ & $3.0_{-1.1}^{+3.8}$   &   71.0, 98.0, 100.0    &   14.0, 33.0, 58.0  &   67.0, 95.0, 100.0   &    4.0, 30.0, 49.0  \\[3pt] 
 40.0  &  37.1 &  $35.9_{-14.7}^{+19.5}$ & $12.1_{-6.4}^{+6.4}$  &    10.3 & 69.8   &    $1.1_{-0.4}^{+0.8}$ & $3.3_{-1.2}^{+3.8}$   &   73.0, 99.0, 99.0    &   6.0, 31.0, 52.0  &   65.0, 93.0, 100.0   &    2.0, 22.0, 45.0  \\[3pt] 
\enddata 
\tablecomments{Uncertainties correspond to the 68.3\% credible or confidence intervals.  Correction factors $\hat{f}_{\mathrm{calc}}$ and $\hat{f}_{\mathrm{calc}}$ are calculated by dividing the true rate by $\hat{\theta}_{\mathrm{calc}}$ and $\hat{\theta}_{\mathrm{detect}}$, respectively. $\epsilon_{\text{calc}}$  and  $\epsilon_{\text{calc}}$  are the percent errors of the calculated occurrence rate and the detection rate with respect to the true rate.}
\end{deluxetable*} 
 
